Calculational Verification of Reactive Programs with Reactive Relations and Kleene Algebra

Reactive programs are ubiquitous in modern applications, and so verification is highly desirable. We present a verification strategy for reactive programs with a large or infinite state space utilising algebraic laws for reactive relations. We define novel operators to characterise interactions and state updates, and an associated equational theory. With this we can calculate a reactive program's denotational semantics, and thereby facilitate automated proof. Of note is our reasoning support for iterative programs with reactive invariants, which is supported by Kleene algebra. We illustrate our strategy by verifying a reactive buffer. Our laws and strategy are mechanised in Isabelle/UTP, which provides soundness guarantees, and practical verification support.

==> circus-rc.tex <==
In this section we specialise our reactive contract theory to allow modelling and calculation of basic \Circus
actions. We will consider external choice in Section~\ref{sec:ext-choice} as it requires special treatment. Whilst
Theorems~\ref{thm:rc-comp} and \ref{thm:rc-iter} show us how to calculate composite contracts, we need further laws to
calculate the underlying relational compositions to support our proof strategy. We must, therefore, specialise our
language of reactive relations for \Circus, and prove theorems for composition with respect to $\relsemi$ and other
operators. These operators give rise to a pattern for reactive relations, and thus facilitate proof automation.

Healthiness condition $\healthy{NCSP} \defs \healthy{NSRD} \circ \healthy{CSP3} \circ \healthy{CSP4}$ characterises
\Circus actions. $\healthy{CSP3}$ and $\healthy{CSP4}$ ensure that well-formedness of the refusal
sets~\cite{Cavalcanti&06,Hoare&98}. \healthy{NCSP}, like \healthy{NSRD}, is continuous and has the $\Skip$ action,
defined below, as a left and right unit. Thus, $(\theoryset{NCSP}, \intchoice, \Miracle, \relsemi, \Skip, \bm{\star})$
forms a Kleene algebra. An \healthy{NCSP} contract has the following specialised form.
%
$$\rc{P(\trace, \state)}{Q(\trace, \state, ref')}{R(\trace, \state, \state')}$$
%
The underlying reactive relations capture a portion of the \Circus stateful failures-divergences
semantics~\cite{Cavalcanti&06,Oliveira&09}. $P$ captures the initial states and traces that do not induce
divergence. $Q$ captures the stateful failures of an action: the set of events not being refused ($ref'$) having
performed trace $\trace$, starting in state $\state$. Finally, $R$ captures the terminated behaviours, where a final
state is observed but no refusals. All contracts for \Circus actions follow a particular pattern, which we will capture
using the following constructs.
%
\begin{definition}[\Circus Reactive Relational Operators]
\begin{align*}
  \cspin{b(\state)}{t(st)} \defs~~ & \healthy{RR}(b(st) \land t(\state) \le \trace) \\
  \cspen{b(\state)}{t(st)}{E(st)} \defs~~ & \healthy{RR}(b(\state) \land \trace = t(\state) \land (\forall e \in E(\state) @ e \notin ref')) \\
  \csppf{b(\state)}{\sigma}{t(st)} \defs~~ & \healthy{RR}(b(\state) \land \state' = \sigma(\state) \land \trace = t(\state))
\end{align*}
\end{definition}

\noindent $\cspin{b(\state)}{t(\state)}$ is a specification of initial behaviour which will be used in preconditions. It
states that initially the state satisfies predicate $b$, and the trace $t$ is a prefix of the overall behaviour, both of
which are expressions in undashed state variables only. $\cspen{b(\state)}{t(\state)}{E(\state)}$ specifies that the
state initially satisfies $b$, the interaction described by $t$ occurred, and finally none of the events in $E$ are
being refused. It will be used in periconditions to specify quiescent observations, where an interaction has occurred
and we are waiting for events in $E$. It corresponds to a failure in CSP. $\csppf{b(\state)}{\sigma}{t(\state)}$
specifies that the initial state satisfies $b$, the state updates described by state substitution $\sigma$ are applied,
and the interaction $t$ has occurred. It is used to encode final observations in the postcondition.

These operators are all deterministic, in the sense that they describe a single interaction and state update
history. There is no need for explicit nondeterminism here, as this is achieved using $\bigsqcap$. These operators allow
us to concisely specify the basic operators of \Circus as given below.

\begin{definition}[Basic \Circus Operators]
\begin{align*}
  \Skip             =& \rc{\true}{\false}{\csppf{\ptrue}{id}{\langle\rangle}} \\[1ex]
  \Stop             =& \rc{\true}{\cspen{\ptrue}{\langle\rangle}{\emptyset}}{\false} \\[1ex]
  \assignsC{\sigma} =& \rc{\true}{\false}{\csppf{\ptrue}{\sigma}{\langle\rangle}} \\[1ex]
  \ckey{Do}(a)      =& \rc{\true}{\cspen{\ptrue}{\langle\rangle}{\{a\}}}{\csppf{\ptrue}{id}{\langle a \rangle}} % \\[1ex]
  % \begin{array}{c}
  %   \rc{P_1}{P_2}{P_3} \\ 
  %   \extchoice \\
  %   \rc{Q_1}{Q_2}{Q_3}
  % \end{array} =& \rc{P_1 \land Q_1}{
  %                  \begin{array}{l}
  %                    (P_2 \land Q_2) \\
  %                    \infixIf \trace = \langle\rangle \infixElse \\
  %                    P_2 \lor Q_2
  %                  \end{array}}{P_3 \lor Q_3} \\[.5ex]
  % g \guard \rc{P}{Q}{R} = & \rc{\cspin{g}{\langle\rangle} \implies P}{\rasm{g} \relsemi Q \lor \cspen{\neg g}{\langle\rangle}{\emptyset}}{\rasm{g} \relsemi R} \\[2ex]
\end{align*}
\end{definition}

% $\assignsr{\sigma}$ is a generalised assignment
% operator, inspired by Back's work, which lifts a substitution function on state, $\sigma : \Sigma \to \Sigma$, to a
% reactive relation, and is defined to be $(\trace = \langle\rangle \land st' = \sigma(st))$. A traditional assignment
% $x := v$ can then be expressed with the substitution $(\lambda s @ s(x \mapsto v))$ which applies an update to incoming
% state $s$.

\noindent These are not definitions, but theorems of the original \Circus definitions~\cite{Oliveira&09,Foster17c}. The
$\Skip$ action has a $\true$ precondition and a $\false$ pericondition, as it has no intermediate observations. The
postcondition uses the $\Phi$ operator to state that for every initial state ($true$) the state remains unchanged
($id$), and no events are produced ($\langle\rangle$). The $\Stop$ action's pericondition states that in any initial
state, the trace is unchanged and no events are being accepted: a deadlock situation. The postcondition is false as
there is no way to reach a final state. 

The generalised assignment operator $\assignsC{\sigma}$ takes inspiration from Back's refinement
calculus~\cite{Back1998}. It is similar to $\Skip$, but applies the state function $\sigma : \Sigma \to \Sigma$ to
update $\state$. A singleton assignment $x := v$ can be expressed using a state update
$\lambda s @ s \oplus \{x \mapsto v\}$. Characterisation of assignments as state updates enables algebraic laws to
variously manipulate them. We can also apply state updates as substitutions on \Circus actions and predicates using
operator $\sigma \dagger P$.

The $\ckey{Do}(a)$ operator encodes an event action, and is equivalent to $a \then \Skip$. Its pericondition states that
when no event has occurred, $a$ is being accepted, and its postcondition extends the trace by $a$, whilst leaving the
state unchanged. The more general event prefix $a \then P$ can be encoded using sequential composition
$\ckey{Do}(a) \relsemi P$. Moreover, the guard operator can be encoded as
$g \guard P \defs (\conditional{P}{g}{\Stop})$, which behaves as $P$ when $g$ is true, and otherwise deadlocks.

In order to calculate and simplify the semantics of a \Circus action, we need laws to reduce pre-, peri-, and
postconditions. These need to cater for the different composition cases that exist for operators $\bigsqcap$,
$\relsemi$, and $\Extchoice$. We prove the following composition laws for $\mathcal{E}$ and $\Phi$.

\begin{theorem}[\Circus Relational Compositions]
  \begin{align}
    \rasm{b} \relsemi P =~~& \csppf{b}{id}{\langle\rangle} \relsemi P \label{thm:crc1} \\[1ex]
    \csppf{b_1}{\sigma_1}{t_1} \relsemi \csppf{b_2}{\sigma_2}{t_2} =~~& \csppf{b_1 \land \substapp{\sigma_1}{b_2}}{\sigma_2 \circ \sigma_1}{t_1 \tcat \substapp{\sigma_1}{t_2}} \label{thm:crc2} \\[1ex]
    \csppf{b_1}{\sigma_1}{t_1} \relsemi \cspen{b_2}{t_2}{E} =~~& \cspen{b_1 \land \substapp{\sigma_1}{b_2}}{t_1 \tcat \substapp{\sigma_1}{t_2}}{\substapp{\sigma_1}{E}} \label{thm:crc3} \\[1ex]
    \conditional{\csppf{b_1}{\sigma_1}{t_1}}{c}{\csppf{b_2}{\sigma_2}{t_2}} =~~& \csppf{\conditional{b_1\!}{\!c\!}{\!b_2}}{\conditional{\sigma_1\!}{\!c\!}{\!\sigma_2}}{\conditional{t_1\!}{\!c\!}{\!t_2}} \label{thm:crc4} \\[1ex]
    \conditional{\cspen{b_1}{t_1}{E_1}}{c}{\cspen{b_2}{t_2}{E_2}} =~~& \cspen{\conditional{b_1\!}{\!c\!}{\!b_2}}{\conditional{t_1\!}{\!c\!}{\!t_2}}{\conditional{E_1\!}{\!c\!}{\!E_2}} \label{thm:crc5} \\[1ex]
    \left(\bigwedge_{i \in I}\,\cspen{b(i)}{t}{E(i)}\right) =~~& \cspen{\bigwedge_{i \in I}\,b(i)}{t}{\bigcup_{i \in I}\,E(i)} \label{thm:crc6}
  \end{align}
\end{theorem}

\noindent Law \ref{thm:crc1} states that a precomposed assumptions can be expressed using the $\Phi$ operator. Law
\ref{thm:crc2} states that the composition of two terminated observations results in the conjunction of the state
conditions, composition of the state updates, and concatenation of the traces. Additionally, it is necessary to apply
the initial state update $\sigma_1$ as a substitution to both the second state condition ($s_2$) and the trace
expression ($t_2$). Law~\ref{thm:crc3} is similar, but accounts for the enabled events rather than state
updates. Laws~\ref{thm:crc2} and \ref{thm:crc3} are required because of Theorem~\thmeqref{thm:rc-comp}{thm:rc-seq},
which sequentially composes a pericondition with a postcondition, and a postcondition with a
postcondition. Laws~\ref{thm:crc4} and \ref{thm:crc5} shows how a conditional distributes through the
operators. Finally, Law \ref{thm:crc6} shows that a conjunction of several intermediate observations which agree on the
trace takes the conjunction of the state conditions, and the union of the enabled events. This is needed due to external
choice, which conjoins the periconditions when the trace is empty (see Section~\ref{sec:ext-choice}).

In order to calculate preconditions for \Circus contracts, we also need to consider reactive weakest
preconditions. Theorem~\thmeqref{thm:rc-comp}{thm:rc-seq} requires that, in a composition, we need to show that the
postcondition satisfies the precondition. Since postconditions can be expressed as nondeterministic choices of the
$\Phi$ operator, we will calculate its weakest precondition.
%
\begin{theorem}[Event Weakest Precondition]
  \begin{align*}
    \csppf{s}{\sigma}{t} \wpR P ~=~& (\cspin{s}{t} \implies (\substapp{\sigma}{P})[\trace - t/\trace])
  \end{align*}
\end{theorem}
%
This law states that, in order for $\csppf{s}{\sigma}{t}$ to satisfy reactive condition $P$, whenever we start in the
state satisfying $s$ and the trace $t$ has been performed, $P$ must hold on the remainder of the trace ($\trace - t$),
and with the state update $\sigma$ applied. We can now use these laws, along with Theorem \ref{thm:rc-comp}, to
calculate the semantics of processes, and to prove equality and refinement conjectures, as we illustrate below.

\begin{example}[Assignment and Prefix]
  $$x := 1 \relsemi a \then x := x + 2 = a \then x := 3$$
\end{example}

\begin{proof} 
  Both sides evaluate to the reactive contract
  $$\rc{\true}{\cspen{true}{\langle\rangle}{\{a\}}}{\csppf{true}{\{x \mapsto 3\}}{\langle a \rangle}}$$ which has a 
  single quiescent state, where we are waiting for an $a$, and a single final state, where $a$ has occurred and state
  variable $x$ has been updated to $3$. They are therefore equivalent. \qed
\end{proof}

\noindent We can also use calculational theorems, with the help of our proof strategy in \textsf{rdes-eq}, to prove a
number of sequential \Circus programming laws~\cite{Oliveira&09}.

\begin{theorem}[\Circus Laws]
  \begin{align}
  \Stop \relsemi P &= \Stop \\
  false \guard P &= \Stop \\
  true  \guard P &= P \\
  b \guard c \guard P &= (b \land c) \guard P \\
  x := v \relsemi e \then P &= e[v/x] \then (x := v \relsemi P) \\
  a \then (P \intchoice Q) &= (a \then P) \intchoice (a \then Q) 
  \end{align}
\end{theorem}

\begin{proof} By application of \textsf{rdes-eq}. \qed \end{proof}

\section{External Choice and Productive Contracts}
\label{sec:ext-choice}

In this section we consider the calculation of actions with external choice, and characterise the important subclass of
productive contracts, which will also be essential in verifying recursive and iterative reactive programs.

An external choice $P \extchoice Q$ resolves whenever either $P$ or $Q$ engages in an event or terminates. Thus, its
semantics requires that we distinguish observations with a non-empty trace. We introduce a healthiness condition,
$\healthy{R4}(P) \defs (P \land \trace > \langle\rangle)$, whose fixed points always strictly increase the trace. We
also introduce its dual $\healthy{R5}(P) \defs (P \land \trace = \langle\rangle)$ where the trace is unchanged. We then
use these functions in our definition of indexed external choice.
%
\begin{align*}
& \Extchoice i \in I @ \rc{P_1(i)}{P_2(i)}{P_3(i)} = \\[1ex]
& \qquad \rc{\bigwedge_{i \in I} P_1(i)}{\left(\bigwedge_{i \in I} \healthy{R5}(P_2(i))\right) \lor \left(\bigvee_{i \in I} \healthy{R4}(P_2(i))\right)}{\bigvee_{i \in I}{P_3(i)}}
\end{align*}
%
As for internal choice (Theorem~\ref{thm:rc-comp}(\ref{thm:rc-choice})), the precondition requires that all constituent preconditions are satisfied. In the
pericondition, we use \healthy{R4} and \healthy{R5} to filter all observations. We take the conjunction of all \ckey{R5}
behaviours, where the trace remains the same. This is because until one of the branches resolves, effectively all
branches are active and waiting to communicate with the environment. We then also take the disjunction of all \ckey{R5}
behaviours, which means that an event has occurred and thus the choice is resolved. In the postcondition the choice must
also have been resolved, either by communication or termination, and thus we take the disjunction of all constituent
postconditions. Since our external choice support unbounded nondeterminism, it can be used to also represent the input
prefix operator of \Circus.

We next show how \healthy{R4} and \healthy{R5} filter the various reactive relational operators, which can be applied to
simplify action contracts involving external choice.
%
\begin{theorem}[Trace Filtering]

\vspace{1ex}
\begin{tabular}{cc}
$\begin{aligned}
  \healthy{R4}\left(\bigvee_{i \in I} P(i)\right) & = \bigvee_{i \in I} \healthy{R4}(P(i)) \\[1ex]
  \healthy{R4}(\csppf{s}{\sigma}{\langle \rangle}) & = \false \\[1ex]
  \healthy{R4}(\csppf{s}{\sigma}{\langle a, ... \rangle}) & = \csppf{s}{\sigma}{\langle a, ... \rangle}
\end{aligned}
\qquad
\begin{aligned}
  \healthy{R5}\left(\bigvee_{i \in I} P(i)\right) & = \bigvee_{i \in I} \healthy{R5}(P(i)) \\[1ex]
  \healthy{R5}(\cspen{s}{\langle \rangle}{E}) & = \cspen{s}{\langle \rangle}{E} \\[1ex]
  \healthy{R5}(\cspen{s}{\langle a, ... \rangle}{E}) & = \false
\end{aligned}$
\end{tabular}
\end{theorem}
%

\begin{example}[External Choice Calculation]
Consider, then, the calculation of the action $a \then b \then \Skip \extchoice c \then \Skip$. The left-hand action has
two quiescent observations, one where it is waiting for $a$, and one where it is waiting for $b$ having performed
$a$. Thus, its pericondition is $\cspen{true}{\langle \rangle}{\{a\}} \lor \cspen{true}{\langle a \rangle}{\{b\}}$.
Application of \healthy{R5} to this will yield the first disjunct, since the trace has not increased, and \healthy{R4}
will yield the second disjunct. For the right-hand side there is only one quiescent observation,
$\cspen{true}{\langle \rangle}{\{c\}}$, which contributes an empty trace and is therefore $\healthy{R5}$ only. The
overall pericondition of the choice is therefore
$$(\cspen{true}{\langle \rangle}{\{a\}} \land \cspen{true}{\langle \rangle}{\{c\}}) \lor \cspen{true}{\langle a
  \rangle}{\{b\}}$$
which is simply $\cspen{true}{\langle \rangle}{\{a, b\}} \lor \cspen{true}{\langle a \rangle}{\{b\}}$. \qed
\end{example}

\noindent By calculation we can now prove that $(\theoryset{NCSP}, \extchoice, \Stop)$ forms a
commutative and idempotent monoid, and $\Chaos$ is its annihilator. Sequential composition also distributes from the
right through external choice, but only in restricted circumstances, specifically when the choice branches are
\emph{productive}.
%
\begin{definition}
  A contract $\rc{P_1}{P_2}{P_3}$ is productive when $P_3$ is \healthy{R4} healthy.
\end{definition}
%
\noindent A productive contract is one which, whenever it terminates, strictly increases the trace. For example
$a \then \Skip$ is productive, but $\Skip$ is not. Constructs which do not terminate at all, like $\Chaos$ and
$\Miracle$, are also productive. We then define the healthiness condition $\healthy{PCSP}$, which extends
$\healthy{NCSP}$ with productivity. As a dual we also define $\healthy{ICSP}$ which requires that the postcondition is
\healthy{R5} healthy and the pericondition is $\false$. For example both $\Skip$ and $x := v$ are $\healthy{ICSP}$
healthy as they do not contribute to the trace and have no intermediate observations. This allows us to state and prove
the following distributivity laws.

\begin{theorem}[External Choice Distributivity]
  \begin{align*}
    (\Extchoice i\!\in\!I @ P(i)) \relsemi Q &~=~ \Extchoice i\!\in\!I @ (P(i) \relsemi Q) & ~~[\text{if, } \forall i\!\in\!I, P(i) \text{ is } \healthy{PCSP} \text{ healthy}] \\[1ex]
    P \relsemi (\Extchoice i\!\in\!I @ Q(i)) &~=~ \Extchoice i\!\in\!I @ (P \relsemi Q(i)) & ~~[\text{if } P \text{ is } \healthy{ICSP} \text{ healthy}]
  \end{align*}
\end{theorem}

\noindent The first law follows because every $P(i)$, being productive, must resolve the choice before terminating, and
thus it is not possible to reach $Q$ before this occurs. The second follows for the converse reason: since $P$ cannot
resolve the choice with any of its behaviour, it is safe to execute it first. 

Productivity also forms an important criterion for guarded recursion that we will utilise in Section~\ref{sec:iter} to
aid in calculating fixed points for iterative actions. We can show that \healthy{PCSP} is closed under several of the
\Circus operators.

\begin{theorem}[Productivity Theorems]
  \begin{itemize}
    \item $\Miracle$, $\Chaos$, $\Stop$, and $\ckey{Do}(a)$ are all \healthy{PCSP} healthy;
    \item $b \guard P$ is \healthy{PCSP} if $P$ is \healthy{PCSP};
    \item $P \relsemi Q$ is \healthy{PCSP} if either $P$ or $Q$ is \healthy{PCSP};
    \item $\Intchoice i \in I @ P(i)$ is \healthy{PCSP} if, for all $i \in I$, $P(i)$ is \healthy{PCSP};
    \item $\Extchoice i \in I @ P(i)$ is \healthy{PCSP} if, for all $i \in I$, $P(i)$ is \healthy{PCSP}.
  \end{itemize}
\end{theorem}

